PG-SELD: Physics-Guided Sound Event Localization and Detection

Sound event localization and detection (SELD) aims to jointly recognize sound events and estimate their directions of arrival from multichannel audio. Although recent deep learning approaches have achieved strong performance, their ability to generalize across acoustic environments remains limited, as room reverberation introduces environment-specific characteristics into the learned representations. In this work, we address this challenge by leveraging a physical free-field model as a room-independent reference. Specifically, we propose PG-SELD, a training framework that combines free-field with physics-guided knowledge distillation. Our approach aligns intermediate representations extracted from reverberant signals with those produced by a free-field teacher for matched acoustic scenes. This guidance encourages the model to preserve event- and localization-relevant information while reducing sensitivity to room-specific characteristics. Experimental results on the STARSS23 benchmark show that PG-SELD consistently improves the generalization performance of multiple baseline SELD architectures.

==> images/room_figure.tex <==

% Room geometry.
\begin{figure}[!t]
    \centering
\begingroup
    \setlength{\fboxsep}{8pt}%
    \resizebox{0.8\columnwidth}{!}{%
\colorbox{white}{%
\begin{tikzpicture}[
    font=\sffamily,
    line cap=round,
    line join=round,
    >={Latex[length=2.4mm,width=1.7mm]},
    multipath/.style={
        draw=multipathcolor,
        line width=1.35pt,
        dashed,
        dash pattern=on 5pt off 3pt,
        opacity=0.88,
        -{Latex[length=2.1mm,width=1.5mm]}
    }
]
    % Irregular five-sided room and clipped floor grid.
    \path[fill=roomfill,rounded corners=2pt]
        (0,0) -- (12,0) -- (12,5.5) -- (10.4,7.5) -- (0,7.5) -- cycle;
    \begin{scope}
        \clip (0,0) -- (12,0) -- (12,5.5) -- (10.4,7.5) -- (0,7.5) -- cycle;
        \draw[step=1cm,gray!10,very thin] (0,0) grid (12,7.5);
    \end{scope}

    % Desk placed flush against the right wall, with monitor and chair.
    \path[fill=deskcolor!18,draw=deskcolor,line width=1.1pt,rounded corners=3pt]
        (10.82,2.45) rectangle (11.82,4.75);
    \draw[deskcolor!75!black,line width=2pt] (11.18,3.25) -- (11.18,3.95);
    \path[fill=wallcolor!85,draw=wallcolor,rounded corners=1pt]
        (11.28,3.13) rectangle (11.66,4.07);
    \draw[wallcolor,line width=1pt] (11.18,3.60) -- (11.28,3.60);
    \path[fill=deskcolor!10,draw=deskcolor,line width=1pt]
        (10.25,3.12) arc[start angle=260,end angle=100,x radius=0.42,y radius=0.50]
        -- cycle;
    \node[text=deskcolor!70!black,font=\small\bfseries,rotate=90]
        at (11.35,2.88) {Desk};

    % Central meeting table and four chairs.
    \path[fill=tablecolor!16,draw=tablecolor,line width=1.2pt]
        (6.05,3.55) ellipse[x radius=1.28,y radius=0.70];
    \path[fill=tablecolor!10,draw=tablecolor,line width=1pt,rounded corners=2pt]
        (5.66,2.45) rectangle (6.44,2.78);
    \path[fill=tablecolor!10,draw=tablecolor,line width=1pt,rounded corners=2pt]
        (5.66,4.32) rectangle (6.44,4.65);
    \path[fill=tablecolor!10,draw=tablecolor,line width=1pt,rounded corners=2pt]
        (4.35,3.20) rectangle (4.68,3.90);
    \path[fill=tablecolor!10,draw=tablecolor,line width=1pt,rounded corners=2pt]
        (7.42,3.20) rectangle (7.75,3.90);
    \node[text=tablecolor,font=\small\bfseries] at (6.05,3.12) {Table};

    % Wall-mounted television.
    \path[fill=wallcolor!92,draw=black,line width=1pt,rounded corners=1.5pt]
        (5.45,6.96) rectangle (7.75,7.40);
    \path[fill=blue!22] (5.62,7.06) rectangle (7.58,7.30);
    \node[text=wallcolor,font=\small\bfseries] at (6.60,6.72) {TV};

    % Multipath propagation paths (drawn below the direct path).
    \draw[multipath]
        (9.40,1.70) -- (11.98,4.20) -- (1.15,6.35);
    \draw[multipath]
        (9.40,1.70) -- (10.95,6.81) -- (1.15,6.35);
    \draw[multipath]
        (9.40,1.70) -- (4.55,0.02) -- (0.02,3.45) -- (1.15,6.35);

    % Wall-reflection markers.
    \foreach \p in {(11.98,4.20),(10.95,6.81),(4.55,0.02),(0.02,3.45)}{
        \fill[white] \p circle (2.6pt);
        \draw[multipathcolor,line width=1pt] \p circle (2.6pt);
    }

    % Highlighted direct (central) path.
    \draw[directcolor!18,line width=10pt,opacity=0.72]
        (9.40,1.70) -- (1.15,6.35);
    \draw[directcolor,line width=2.5pt,-{Latex[length=3mm,width=2.1mm]}]
        (9.40,1.70) -- (1.15,6.35);

    % Room walls.
    \draw[wallcolor,line width=3.2pt,rounded corners=2pt]
        (0,0) -- (12,0) -- (12,5.5) -- (10.4,7.5) -- (0,7.5) -- cycle;

    % Hinged door placed next to the lower-right corner.
    \draw[roomfill,line width=4.8pt] (10.38,0) -- (11.80,0);
    \draw[wallcolor,line width=1.6pt] (10.38,0) -- (10.38,1.42);
    \draw[wallcolor!55,line width=0.9pt,dashed]
        (11.80,0) arc[start angle=0,end angle=90,radius=1.42];
    \fill[wallcolor] (10.38,0) circle (2.2pt);
    \node[text=wallcolor,font=\small\bfseries] at (11.12,0.47) {Door};

    % Four-microphone cross array near the upper-left corner.
    \draw[arraycolor!24,line width=8pt]
        (0.70,6.35) -- (1.60,6.35)
        (1.15,5.90) -- (1.15,6.80);
    \draw[arraycolor,line width=1.5pt]
        (0.70,6.35) -- (1.60,6.35)
        (1.15,5.90) -- (1.15,6.80);
    \foreach \mic in {(0.70,6.35),(1.60,6.35),(1.15,5.90),(1.15,6.80)}{
        \fill[white] \mic circle (4pt);
        \draw[arraycolor,line width=1.4pt] \mic circle (4pt);
        \fill[arraycolor] \mic circle (1.45pt);
    }
    \fill[arraycolor] (1.15,6.35) circle (1.8pt);
    \node[anchor=south west,text=arraycolor,font=\bfseries]
        at (0.35,7.02) {Microphone Array};

    % Speaking person, shown from above.
    \begin{scope}[shift={(9.40,1.70)}]
        \fill[personcolor!13] (0,0) circle (0.54);
        \draw[personcolor,line width=1.5pt] (0,0.13) circle (0.18);
        \draw[personcolor,line width=1.5pt]
            (-0.34,-0.34) .. controls (-0.25,-0.04) and (0.25,-0.04) .. (0.34,-0.34);
        \draw[personcolor,line width=1.25pt]
            (-0.36,0.13) arc[start angle=180,end angle=360,radius=0.36];
        \draw[personcolor,line width=1.2pt]
            (-0.45,0.30) arc[start angle=135,end angle=215,radius=0.22];
        \draw[personcolor,line width=1.2pt]
            (-0.56,0.39) arc[start angle=135,end angle=215,radius=0.38];
    \end{scope}
    \node[below=7pt,text=personcolor,font=\bfseries] at (9.40,1.15) {Speaker};

    % Path labels.
    \node[
        fill=white,
        inner sep=3pt,
        text=directcolor,
        font=\bfseries,
        rotate=-29
    ] at (4.15,4.67) {Direct path};
    \node[
        fill=white,
        rounded corners=2pt,
        inner sep=4pt,
        text=multipathcolor,
        font=\bfseries
    ] at (9.25,6.18) {Reflected multipath};
\end{tikzpicture}
}%
    }
\endgroup
    \caption{A reverberant room containing a microphone array, a source,
    and direct and reflected propagation paths.}
    \label{fig:room-geometry}
\end{figure}
